Convex Parameterizations and Fidelity Bounds for Nonlinear Identification and Reduced-Order Modelling

Model instability and poor prediction of long-term behavior are common problems when modeling dynamical systems using nonlinear "black-box" techniques. Direct optimization of the long-term predictions, often called simulation error minimization, leads to optimization problems that are generally non-convex in the model parameters and suffer from multiple local minima. In this work we present methods which address these problems through convex optimization, based on Lagrangian relaxation, dissipation inequalities, contraction theory, and semidefinite programming. We demonstrate the proposed methods with a model order reduction task for electronic circuit design and the identification of a pneumatic actuator from experiment.

==> tacConc.tex <==
In this paper, we have introduced techniques for convex parameterization
of nonlinear models, together with a family of upper bounds of
simulation error, for use in nonlinear model reduction and system identification. The Lagrangian relaxation is most accurate, but may
be prohibitively expensive to compute. Dissipation
inequalities and linearized simulation error were introduced to simplify the optimization problems, resulting in the RIE and local RIE respectively.
The local RIE was shown to be effective on two real-world problems of model reduction and system identification.

%We have provided a number of specific algorithms for model identification, however it is clear that the general methodology proposed admits many variations. Natural directions for future research include different formulations of
%multipliers, storage functions, and surrogate state sequences, as well as cost functions incorporating statistical models of noise or disturbance.

==> tacIntro.tex <==
Building approximate models of dynamical systems from data is a ubiquitous task in the sciences and engineering. Reduced order modelling and system identification are two well-known cases, which differ mainly in the source of the data. In reduced order modelling the data come from simulation ``snapshots'' of a complex model, which is usually based on physical principles \cite{willcox2002balanced, Lall02, lucia2004reduced, pedro2005comparative}. The major problem is finding a model that simulates accurately despite unmodelled dynamics. In system identification the data come from experimental recordings \cite{Sjoberg95, Ljung99, pearson2006nonlinear, Ljung10}, and in addition to unmodelled dynamics there are usually the problems of measurement noise and exogenous disturbances.
% COMMENT(mmt): Hankel, BT, and modal MOR does not involve discrete measurements.  Maybe "empirical model order reduction" or some other term is more appropriate?
% IRM - Maybe we should mention, here or elsewhere, that many MOR methods take the model equations as input data, not simulation data...

Another class of model reduction algorithms work directly from the defining equations of the high-order model rather than simulation snapshots, e.g. balanced truncation and Hankel-optimal reduction  (see, e.g., \cite{antoulas2005approximation}, \cite{fujimoto2010balanced} and references therein). We do not consider this problem here.

The basic objective we consider is to obtain a causal system that reliably reproduces the observed relationship between between some given input data $\tilde u(t)\in\RR^m$ and output data $\tilde y(t)\in\RR^p$, for $t = 0, 1, 2, ..., T$.  A complete solution using optimization methods requires a specification of a model class, a choice of objective function, and an algorithm for minimizing the objective function over the model class.
% COMMENT(mmt):  This paragraph sort of glosses over the issue of generalization to new inputs... thoughts?
% IRM - good point to mention stability (as is done later)... I'll think about wording.

The main contributions of this paper are a class of nonlinear models that is convex in its parameters and guarantees stability, and a family of convex upper bounds for minimization of simulation error. The combination of these allows problems in reduced order modelling and identification to be approached using semidefinite programming. This paper unifies and extends work of the authors and colleagues that was presented in a series of conference papers \cite{Megretski08}, \cite{tobenkin2010convex}, \cite{manchester2012stable}, and the applications paper \cite{Bond10}. In this paper, we do not investigate the effects of measurement noise, but we note that a modified version of the proposed method gives consistent estimates when repeated noisy measurements are available \cite{manchester2012stable, tobenkin2013stable}.

\subsection{Classes of Nonlinear Models}

Perhaps the most widely used nonlinear model classes represent the output at time $t$ as an explicit function of the input history:
\begin{equation}\label{eq:iomap}
y(t) = F_{d}(u(t),  u(t-1), u(t-2), ... )
\end{equation}
or, more practically, some finite truncation of the input history \cite{Sjoberg95, pearson2006nonlinear, lucia2004reduced, pedro2005comparative}. 

When based on a finite truncation, such models are often referred to as Nonlinear Finite Impulse Response (NFIR) \cite{Sjoberg95}, and many types of function approximators have been applied. 
The Volterra and Wiener series, for example, represent $F_{d}$ as a finite polynomial expansions of the input history \cite{schetzen1980volterra, Doyle02}, and other popular options include artificial neural networks or wavelets. Non-parametric models based on kernel methods \cite{pillonetto2011new} or direct weight optimization \cite{Roll05} do not in principle depend on a fixed truncation, but grow in evaluation complexity as the amount of data increases. The benefits and drawbacks of direct model structures are well known: model fitting is usually straightforward and models are always stable, but they are typically very inefficient at capturing highly nonlinear or resonant behaviour. 
% COMMENT(mmt): Maybe this and the above should be a single paragraph? IRM - done.

%Nevertheless, there are disadvantages of models of the form \eqref{eq:iomap}. When the system to be modeled exhibits resonance or very slow decay rate, input/output models require a very large number of parameters or data points, especially when there is also substantial nonlinearity present. These problems can be alleviated to some degree by choice of basis functions \cite{da2007choice} or kernel descriptions \cite{pillonetto2011new}, but the resulting optimizations are generally nonconvex.



Such inherently dynamic behaviour can be represented more compactly by models with {\em feedback}, e.g. autoregressive or state-space models. For example, Wiener and Hammerstein models consist of cascades of linear dynamic systems and nonlinear static functions \cite{narendra1966iterative, billings1982identification, bai1998optimal}. Other model structures incorporate {\em nonlinear} feedback, for example nonlinear autoregressive models:
\begin{equation}\label{eq:NARX}
y(t) = F_{ar}(y(t-1),  y(t-2), ... , u(t), u(t-1), ... ),
\end{equation}
where the function $F_{ar}$ can again take a variety of forms, e.g. polynomial, wavelet, neural network \cite{Sjoberg95} or non-parametric kernels \cite{bai2007identification, pillonetto2011new}. Many models considered in the system identification literature consist of \eqref{eq:NARX} with the addition of a statistical model of noise, e.g. NARX, NARMAX \cite{Sjoberg95, billings2013nonlinear}. 
The inclusion of feedback in a model of course means that stability is no longer guaranteed, and in the majority of applications an unstable model would be unacceptable. 
% COMMENT(mmt): Similarly, maybe this and the above should be a single paragraph?

In this paper we construct nonlinear state space models of the form
\begin{equation}\label{eq:nlss}
x(t+1) = a(x(t),  u(t)), \ \ y(t) = g(x(t),  u(t)).
\end{equation}
Note that this class includes models of the form \eqref{eq:NARX} by choosing the states to be $x(t) = [ y(t)', y(t-1)', y(t-2)', ... , y(t-s)']'$ for some integer $s$ and the vector $u(t)$ as a virtual input consisting of a stacked history of true inputs. Nonlinear state-space models have been studied in the context of model reduction \cite{Lall02, rewienski2003trajectory} and system identification \cite{Schon10}.

We consider $a$ and $g$ to be ``black boxes''. When some known structure can be incorporated into a model it is usually preferable to do so, but black-box modeling
plays an important role when first-principles models are either
weakly identifiable, too complicated for the eventual application, or
simply unavailable (see, e.g. \cite{Sjoberg95, Ljung99, Ljung10}).  In many applications, it is important that $a(\cdot, \cdot),  g(\cdot, \cdot)$ are ``simple'' functions that are not computationally expensive to evaluate.

Ensuring stability of models with feedback is a significant problem and has been studied for many years, although primarily for linear systems \cite{pearson2006nonlinear, Ljung10}. It is known that linear autoregressive models fit using equation error are stable if the input is generated by an autoregressive process and the data sequence is sufficiently long \cite{Regalia95}.  Jury criteria for stability were enforced in  \cite{Nallasivam11}, and LMI relaxations thereof in \cite{cerone2011enforcing}.
% COMMENT(mmt): autoregressive exogenous input (ARX)?  or linear autogressive models?
% COMMENT(mmt): Maybe say "fitting models by the equation error method"? or Least squares.  Do they really refer to their spectral constraints as stationarity constraints? 
% The ARX comment seems a bit unclear -- maybe 

Stability of linear state space models generated by subspace identification was studied in \cite{maciejowski1995guaranteed}, where it was noted that stability can be enforced by inserting blocks of zeros in the shifted state matrix. In \cite{van2001identification} stability was imposed via regularization, while LMI parametrizations of stable models were given in \cite{Lacy03}. In \cite{miller2013subspace}, a similar method allowed pole locations to be constrained to polytopic convex sets using the formulation in \cite{chilali1996h}.

To the authors knowledge, there are few published results on enforcing stability of nonlinear identified models. Of note is the fact that nonparametric kernels of the form \eqref{eq:iomap} can be forced to be stable by imposing a certain ``decay'' over time on the influence of past values of $u$ \cite{pillonetto2011new}. In \cite{besselink2012model, besselink2013model} small-gain and passivity-like stability guarantees were given for reduction of a high-order linear system in feedback with a convergent nonlinear system.


\subsection{Optimization Criteria for Model Identification}

Given a set of models, one must specify how to rank different candidate models against the data. There are many possibilities, but perhaps the most natural and straightforward measure of quality is {\em simulation error}, also known as {\em output error}:
\[
J_{se} := \sum_{t=0}^T |y(t)-\tilde y(t)|^2
\]
where $\tilde y(t)$ is the output data from the true system, $y(t)$ is the output of the model simulation, both are driven with the same input $\tilde u(t)$, and initial conditions are not fixed. 

%When the obtained model is to be used for simulation and analysis, or for design of controllers, estimators, or compensitors, it is usually important that the model have a relatively low state dimension, and the functions $a$ and $g$ be simple to evaluate and amenable to systematic design procedures.

Global minimization of $J_{se}$ poses major challenges for models with feedback. E.g., for the state space model \eqref{eq:nlss} the simulation output is generated by the recursion
\[
y(t) = g(a(a(... a(x(0),\tilde u(0)),..., \tilde u(t-1)) , \tilde u(t)).
\]
so even if $a$ and $g$ are linearly parametrized, $J_{se}$ is a highly nonlinear function of the model parameters. Indeed, one can find poor local minima even for the class of second-order linear models  \cite{soderstrom1975uniqueness}.

% COMMENT(mmt): Its been pointed out by reveiwers before that "equation error" usually refers to fitting of input-output models, not state-space models.  Maybe least squares error is safer?
A computationally simpler alternative is to minimize {\em equation error}, i.e.
\[
J_{ee} =\sum_t|\tilde y(t) - F_{ar}(\tilde y(t-1), \tilde y(t-2), ... , \tilde u(t), ... )|^2
\]
for an autoregressive model, or
\begin{align}
J_{ee} := \sum_t&\big(|\tilde x(t+1)-a(\tilde x(t), \tilde u(t))|^2 \notag \\ &+ |\tilde y(t+1)-g(\tilde x(t), \tilde u(t))|^2\big). \label{eq:Jee}
\end{align}
% COMMENT(mmt): Is this the first mention of \tilde x(t)?  Maybe exchanging this formula and the next one with a mention that \tilde x(t) is a state estimate? 
for a state space model. Note that in the latter case a sequence of ``surrogate states'' $\tilde x(t)$ is required, we discuss this further in the next subsection.

% COMMENT(mmt): { --> ( in the sums and this equation is missing |.|^2. IRM - fixed.
Nonlinear ARX and subspace identification, for example, use these criteria \cite{Sjoberg95, Ljung99}. The main advantage is that when the model functions $a, g$ or $F_{ar}$ are linearly parametrized, the minimization amounts to basic least squares and can be solved very efficiently.  The disadvantage is that there is in general no connection between equation error and simulation error, since an unstable (or weakly stable) model might be found for which small equation errors accumulate under recursive simulation.

A broader set of criteria can be considered based on prediction error or statistical models \cite{Ljung99}. The prediction error method seeks to minimize the difference between $\tilde y$ and
\begin{equation}\label{eq:onesteppredictor}
\hat y(t) = F_{pe}(\tilde y(t-1), \tilde y(t-2), ... , \tilde u(t), \tilde u(t-1), ... ),
\end{equation}
% Maybe use \hat y(t)  for the LHS of this equation to distinguish from y(t)? IRM - fixed.
where $F_{pe}$ is a predictor or filter for the identified model \cite{Ljung99}. Most statistical methods are based on maximizing the likelihood or a-posteriori probability of parameters \cite{Ljung99, Schon10}, or in some cases estimating a posterior distribution of parameters using Bayesian inference \cite{lindsten2013bayesian}. Both equation error and simulation error can be derived from the maximum likelihood or prediction error methods, by appropriate choice of of noise model or predictor \cite[Ch 7]{Ljung99}.

\subsection{Algorithms for Model Identification}
% COMMENT(mmt): Need to read this section still.

Many algorithms for simulation error minimization work from a sequence of surrogate state data $\tilde x(t)$, either implicitly or explicitly. The use of an autoregressive model structure is based on the implicit assumption that a recent history of outputs provides sufficient information for prediction of future outputs, to some extent justified by Takens' theorem \cite{Kantz97}. 

Explicit methods for generating surrogate states for model reduction include proper orthogonal decomposition \cite{Holmes98} and empirical balanced truncation \cite{Lall02, willcox2002balanced}. In system identification, subspace methods for linear systems are frequently applied \cite{Overschee94}. Extensions of subspace identification have been investigated for identification of nonlinear systems \cite{verdult2000identification}, \cite{Goethals05}. It is not essential that there be a single stage of generating states, followed by a single stage of model fitting. The two can be combined in a nested optimization \cite{Ramsay07} or alternated between using the expectation-maximization algorithm \cite{Schon10}.

Simulation-error minimization is usually approached by first generating an initial set of parameters, e.g. using equation error or related projection methods, and then conducting a local search (e.g. Gauss-Newton) for a locally optimal model \cite{Ljung99}. A recent method proposed to improve convergence is based on successively solving $k$-step prediction problems with increasing $k$, from $k=1$, which is generally convex, until $k=T$ which gives simulation error \cite{farina2011simulation}. However, convergence results remain local in general.

%\subsection{Contributions of This Paper}

%This paper unifies and extends We consider the problem of simulation-error minimization for models with feedback, specifically a class of nonlinear state space models. The main contributions of this paper are a family of finite-dimensional convex parameterizations of stable nonlinear models, and convex upper bounds on simulation error of such models.  

%The bounds we present are valid for finite data sequences, and do not assume that the true system is in the model class.

%Experimental results include identification from real data from a hydrualic pump, and a reduced-order inverse modelling of an electronic circuit.

%Section outline?




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "tacRevised"
%%% End: 


==> tacLinear.tex <==

\subsection{Frequency Domain Interpretation}
\subsection{Tightness of Relaxation}

Multistep and pointwise RIE, transfer function representation.

\subsection{Tightness of Relaxation}

Tightness at a point,

Adaptive update of multiplier

